Multilingual Machine Translation: Closing the Gap between Shared and Language-specific Encoder-Decoders

State-of-the-art multilingual machine translation relies on a universal encoder-decoder, which requires retraining the entire system to add new languages. In this paper, we propose an alternative approach that is based on language-specific encoder-decoders, and can thus be more easily extended to new languages by learning their corresponding modules. So as to encourage a common interlingua representation, we simultaneously train the N initial languages. Our experiments show that the proposed approach outperforms the universal encoder-decoder by 3.28 BLEU points on average, and when adding new languages, without the need to retrain the rest of the modules. All in all, our work closes the gap between shared and language-specific encoder-decoders, advancing toward modular multilingual machine translation systems that can be flexibly extended in lifelong learning settings.

==> implementation.tex <==



==> visualization.tex <==
%congelado

%OLD
%70 votos para lograr la presidencia
%se pudo en parte limitar los daños
%cancer of the breast
%it is also a risk factor
%ses restriccions ne son pas


%new
%recomiendo que se haga el test
%parte el sistema americano
%the American democratic system
%they were able to partially limit the damage
%have adopted laws requiring

%google
%prevenir la enfermedad
%take the test or not
%los productos
%it is also a risk factor
%ses restriccions ne son pas 


As follows, we use a tool \cite{escolano-etal-2019-multilingual} freely available\footnote{https://github.com/elorala/interlingua-visualization} that allows to visualize the intermediate sentences representations. The tool uses the encoder output fixed-representations as input data and makes a dimensionality reduction of these data using UMAP \cite{mcinnes2018umap-software}. We compare the intermediate representation for the three different architectures presented above (shared, basic and frozen). Figures \ref{fig:vis1} and \ref{fig:vis2} show the intermediate representation for XX sentences in all languages (DE, EN, ES, FR and RU) for the 3 configurations under study (shared, basic and frozen). In particular, Figure \ref{fig:vis1} shows the representation for sentence \textit{since 2011 a dozen States have adopted laws requiring voters to prove they are American citizens} and the corresponding translations. Figure \ref{fig:vis2} shows the representation for sentence \textit{en ese sentido, estas medidas minar\'an en parte el sistema democrático americano}. Note that, although all the points seems to be mixed, the representation of the same sentence in different languages is not placed exactly in the same point in the space. For the examples we are showing, representation seems closer for the frozen architecture than in the other two cases. In the case of the basic architecture, the Russian, which is the language that is added later, seems to be quite separated from others.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/visgoogle.png}
    \includegraphics[width=0.5\textwidth]{images/vissincongelado.png}
    \includegraphics[width=0.5\textwidth]{images/viscongelado.png}
    \caption{Visualization 1 for the shared (up), basic (middle) and frozen (bottom) approaches.}
    \label{fig:vis1}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/google2.png}
     \includegraphics[width=0.5\textwidth]{images/singcongelar2.png}
    \includegraphics[width=0.5\textwidth]{images/congelado2.png}
    \caption{Visualization 2 for the shared (up), basic (middle) and frozen (bottom) approaches.}
    \label{fig:vis2}
\end{figure}


{\color{red} add word embedding figures}
